Value-Dependent Session Design in a Dependently Typed Language

Session Types offer a typing discipline that allows protocol specifications to be used during type-checking, ensuring that implementations adhere to a given specification. When looking to realise global session types in a dependently typed language care must be taken that values introduced in the description are used by roles that know about the value. We present Sessions, a Resource Dependent EDSL for describing global session descriptions in the dependently typed language Idris. As we construct session descriptions the values parameterising the EDSLs' type keeps track of roles and messages they have encountered. We can use this knowledge to ensure that message values are only used by those who know the value. Sessions supports protocol descriptions that are computable, composable, higher-order, and value-dependent. We demonstrate Sessions expressiveness by describing the TCP Handshake, a multi-modal server providing echo and basic arithmetic operations, and a Higher-Order protocol that supports an authentication interaction step.

==> eptcsdata.tex <==
\providecommand{\firstpage}{47}
\providecommand{\publicationstatus}{F. Martins, D. Orchard (Eds.): Programming Language Approaches \\
to Concurrency- \& Communication-cEntric Software (PLACES 2019)\\
EPTCS 291, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.291.5}{10.4204/EPTCS.291.5}}
\pdfoutput=1

